Remote Identification Trajectory Coverage in Urban Air Mobility Applications

As Urban Air Mobility (UAM) and Advanced Air Mobility (AAM) continue to mature, a safety-critical system that will need to be implemented in tandem is Remote Identification (Remote ID) for uncrewed aircraft systems (UAS). To ensure successful and efficient deployment (e.g., maximal surveillance of UAS trajectories), as well as to better understand secondary impacts (e.g., consumer privacy risks in collecting real-time UAS trajectory information), the coverage of broadcast-receive Remote ID architectures needs to be characterized. Motivated by this need, we examine theoretical and empirical trajectory coverage of several common Remote ID technologies (e.g., Bluetooth, Wi-Fi) deployed for urban package delivery missions, a commonly-cited use case for UAM and AAM. We derive methods to explicitly compute expected coverage proportions under idealized geometries, as well as conduct case studies with realistic city geographies and UAS path planning algorithms. An example of results include approximate magnitudes of Remote ID receivers needed (approximately 500-5000 receivers needed to achieve 50-95\% coverage for Bluetooth Legacy, and approximately 10-40 receivers needed for the same coverage range for Wi-Fi NAN/Beacon, assuming a cruise altitude of 200 feet) to achieve specific trajectory coverage proportions for San Francisco, California. Our analyses, combined with complementary works related to Remote ID bandwidth and deployment topologies, can help guide municipal authorities and AAM stakeholders in future Remote ID system deployments and upkeep.

==> ridcov_atm2023/chapters/notes_outline.tex <==
Paper outline

I. Introduction % ML
    1. Research Problem/Problem Statement/Research Gap
    2. Motivation
    3. Previous work
        - Advanced Air Mobility (AAM) in general (esp. urban use cases)
        - Remote ID (laws, regs, tech specs)
        - Coverage problems

II. Contribution of Work % ML
    - First analysis of Remote ID coverage for AAM applications
    - Theory + Real world case studies
    - Discuss (high-level) the results/insights

III. Methods and Data % BM, HH, ML
    A. Methods: Idealized analysis and urban area simulations % HH, ML
        a. Idealized analysis % HH
            - Analytical derivations
                1. Circle environment case 
                    - Uniform OD (Case 1)
                    - Uniform midpoint (Case 2)
                2. Square (if time) -- Monte carlo-based simulation only % we will talk square case in Section IV 
            - Description of fixed OD setup
                - Vertiports/etc. are fixed infrastructure
                - Connect random vertiports via paths
        b. Urban area simulations % BM, ML
            - Overview of path planning approaches % BM
                1. Straight path OD
                    - Fly over buildings
                    - Also a lot of other AAM papers assume this (cite Chris, etc.)
                2. Visibility graph (cite Joseph, etc.)
                    - "Shortest path"
                3. RRT* 
                    - Describe briefly and cite due to popularity
            - High-level walkthrough of what pieces you had to get together to start doing the simulation % BM
            - Flowchart of simulation input/output/process % Not priority, ML

    B. Data % subsection may get cut if space comes down to it -- XX
        - System parameters: Remote ID coverage radii, size of the "fake environment"
        - Data for simulation setup
            - Data sets, OSM, Joseph's basemap etc.
            - HIGH LEVEL description

IV. Idealized Coverage Analysis % HH, ML
    %  value over Rc/Re -> Fig 5
    %  Update fixed case: clean fixed
    %  Code
    1. Monte Carlo setup
    2. Comparison between Monte Carlo vs. Analytical
        - For circle environment
        % - For square (if time)
    3. Sensitivity analysis
        - Varying Rd, Re
        - Comparisons between Case 1 and Case 2 as a function of Rd and Re

    4. Simulation-only experiments (no analytical)
        - Square case
            - Describe the setup, and why we conjecture we can approximate it well with the circle case
            - Comparison of simulation square case vs. circle analytical case (inscribed/circumscribed)
        - Fixed OD
            - Provide brief "recall" and summary of the setup (look at section 3)
            - Show results, convergence to true expected proportion
    
    % 4. Walkthrough of fixed OD results (*)
    %     - For square (if time)
    %     - Monte carlo simulation converging to true proportion

V. Urban Area Simulation Case Studies % BM, ML
    1. Data set description -- LOW LEVEL DESCRIPTION/more in-detail
        - Remote ID parameters (radius R1, ..., Rk)
        - Remote ID distribution assumptions (spatial distribution of remote ID sensors DR1, ..., DRn) % Low priority, start with ONE distribution (e.g., uniform)
        - Origin/destination selection (FIXED -- ONLY ONE WAY PER CITY)
        - Base maps and alterations, etc. (different cities, NYC, SFO, etc.)
    2. Case Results
        - Compare within one city, for example, compare across:
            1. (CITY, RID parameter, PP algorithm)
            (NYC, {R,DR}, {SL, VG, RRT})



VI. Concluding Remarks % ML
    1. Limitations of Work
        - Simplifying assumptions made in idealized coverage analysis
        - Simplifying assumptions regarding drone dynamics/simulation/etc.
    2. Future lines of research/future work
        - More realistic implementations, etc.
        - Link with UAV privacy work, which assumed 100\% coverage, we will show some other proportions, so how do you bridge the gap (e.g., predicting rest of trajectory, how accurately can you do so, etc.)
        - Thinking about more path planning/trajectory generation
            - Kinematic feasibility OR
            - Easier to compute, etc.

References and Author Biographies


* Figure 1 2, large font size, remove the unit 1,2,3 (take)
* Correct 3D plot (0.5Re) and (0.79Re), convert 2D plan (take)
* Square case
* setup for Fixed OD, 5 points simulation, pseudo code

==> ridcov_atm2023/hh/bak/2_distribution_of_intpts.tex <==
\section{Distribution}		\label{SEC_Distr}



\subsection{Introduction}

Given a circle-shape sensor region $\mathcal{S}$ in a 2D plane as
$$
\mathcal{S} = \{(x,y);x,y\sim\mathcal{U}(0,1)| (x-x_0)^2+(y-y_0)^2=R^2\},
$$
where $(x_0,y_0)$ is a given center of the sensor region.

Now given 2 points  $O:(x_1,y_1),D:(x_2,y_2)$, the possible intersection point of $\mathcal{S}$ and the line consist of $OD$ 
$$
y = kx +b,
$$
where $k =  \frac{y_2-y_1}{x_2-x_1}$ and $b=\frac{x_2 y_1 - x_1 y_2}{x_2- x_1} $. The related solution is shown below,

$$
x_{sol} = \left(\begin{array}{c} -\frac{2\,b\,k-k+\sqrt{4\,b^2+4\,b\,k-4\,b+\frac{16\,k^2}{25}-2\,k+\frac{34}{25}}+1}{2\,k^2-2}\\ \frac{k-2\,b\,k+\sqrt{4\,b^2+4\,b\,k-4\,b+\frac{16\,k^2}{25}-2\,k+\frac{34}{25}}-1}{2\,k^2-2} \end{array}\right),
$$

$$
y_{sol} = \left(\begin{array}{c} -\frac{2\,b+k-k^2+\frac{\sqrt{2}\,k\,\sqrt{50\,b^2+50\,b\,k-50\,b+8\,k^2-25\,k+17}}{5}}{2\,\left(k^2-1\right)}\\ -\frac{2\,b+k-k^2-\frac{\sqrt{2}\,k\,\sqrt{50\,b^2+50\,b\,k-50\,b+8\,k^2-25\,k+17}}{5}}{2\,\left(k^2-1\right)} \end{array}\right),
$$

\begin{equation}\nonumber
    \begin{aligned}
        I_1 = [x_{{sol}}(1), y_{{sol}}(1)],
    \end{aligned}
\end{equation}

\begin{equation}\nonumber
    \begin{aligned}
    I_2 = [x_{{sol}}(2), y_{{sol}}(2)],
    \end{aligned}
\end{equation}
\noindent
where $I_1$ and $I_2$ are the potential intersection point as given.

\subsection{basic operation of two independent uniform variables}
Consider the random variable that satisfies the following probability density function
\begin{equation}\label{eqn:udist}
    f(x) = \left\{
    \begin{aligned}
        &1 \quad 0<x<1\\
        &0 \quad \text{else}.
    \end{aligned}        
    \right.
\end{equation}
Now, we are given $4$ independent identical variables $x_1,x_2,y_1,y_2$, which satisfy the following rules
\begin{itemize}
    \item Add: $z = x+y$, where $x,y$ satisfy (\ref{eqn:udist}) such that
    \begin{equation}\label{eqn:udistadd}
    f_z(z) = \left\{
    \begin{aligned}
        &z \quad &&0<z<1\\
        &2-z \quad &&1\leq z<2\\
        &0 \quad &&\text{else}.
    \end{aligned}        
    \right.
\end{equation}

\item Sub: $z = x-y$, where $x,y$ satisfy (\ref{eqn:udist}) such that
    \begin{equation}\label{eqn:udistsub}
    f_z(z) = \left\{
    \begin{aligned}
        &z+1 \quad &&-1<z<0\\
        &1-z \quad &&0\leq z<1\\
        &0 \quad &&\text{else}.
    \end{aligned}        
    \right.
\end{equation}

\item Times: $z = xy$, where $x,y$ satisfy (\ref{eqn:udist}) such that
    \begin{equation}\label{eqn:udisttimes}
    f_z(z) = \left\{
    \begin{aligned}
        &-\ln z \quad &&0<z<1\\
        &0 \quad &&\text{else}.
    \end{aligned}        
    \right.
\end{equation}

\item Div: $z = \frac{y}{x}$, where $x,y$ satisfy (\ref{eqn:udist}) such that
    \begin{equation}\label{eqn:udistdiv}
    f_z(z) = \left\{
    \begin{aligned}
        &\frac{1}{2} \quad &&0<z<1\\
        &\frac{1}{2z^2} \quad && z>2\\
        &0 \quad &&\text{else}.
    \end{aligned}        
    \right.
\end{equation}

\item Square: $z = x^2$, where $x$ satisfies (\ref{eqn:udist}) such that
    \begin{equation}\label{eqn:udistsquare}
    f_z(z) = \left\{
    \begin{aligned}
        &\frac{1}{2\sqrt{z}} \quad &&0<z<1\\
        &0 \quad &&\text{else}.
    \end{aligned}        
    \right.
\end{equation}

\item Root: $z = \sqrt{x}$, where $x$ satisfies (\ref{eqn:udist}) such that
    \begin{equation}\label{eqn:udistroot}
    f_z(z) = \left\{
    \begin{aligned}
        &2z \quad &&0<z<1\\
        &0 \quad &&\text{else},
    \end{aligned}        
    \right.
\end{equation}

\end{itemize}



\subsection{Distribution of $k$ and $b$}

Since $(x_2-x_1)$, $(y_2-y_1)$ are standard triangular distributions, thus the distribution of two standard triangular random variables.

==> ridcov_atm2023/hh/bak/2_setting.tex <==
\section{Discussion}\label{SEC_Dis}

Following our discussion above, we are wondering to estimate the length proportion expectation between crossing length of the sensor area and the total length of each RID. But before we formally start our work, some clarifications need to be stated here. 
\begin{itemize}
    \item Circle-shaped sensor region and square-shaped sensor region will be discussed, respectively. 
    \item The orientation and destination of RID is defined with different assumption case by case. But we will sum up to draw a conclusion in the following section. 
\end{itemize}
\noindent
The coverage estimation is demonstrated as shown in Figure \ref{fig:prob_circ} and Figure \ref{fig:prob_squ}. Notice that the definition of random select two points on the target square is ambiguous, which is known as the Bertrand Paradox. So, we will demonstrate all of these situations for both cases in this section, and draw our methodology and conclusions for RID in the next section.

\begin{figure}[t] 
	\centering
	\includegraphics[width=1\linewidth]{figures/prob_demo_circle.eps}
	\caption{RID coverage with circle region}
	\label{fig:prob_circ}
\end{figure}

\begin{figure}[t] 
	\centering
	\includegraphics[width=1\linewidth]{figures/prob_demo_square.eps}
	\caption{RID coverage with square region}
	\label{fig:prob_squ}
\end{figure}

\subsection{Case 1: Circle Region}
Given a set $\mathcal{P}$ containing $n$ points in a 2D-plane as 
$$
\mathcal{P}=\{(x_1,y_1),(x_2,y_2),\dots,(x_n,y_n)\},
$$
while these points are on a circle 
$$
\bigcirc\equiv \{(x,y)| (x-x_0)^2+(y-y_0)^2 = R_1^2\}.$$ 


\subsubsection{Circle Assumption 1}
A special assumption about random endpoints of $L$ is used to generate $\mathcal{P}$ here. 

\begin{asu}
    The chord's endpoints $\mathcal{P}$ of $\bigcirc$ are uniformly distributed on the circumference.
\end{asu}
\noindent
Accordingly, if there exists another endpoint inside a certain range arc, the intersection will happen absolutely.

\begin{figure*}[ht] 
    \centering
    \includegraphics[width=1.0\linewidth]{figures/asp1_demo_circle.eps}
    \caption{Circle case with Assumption 1}
    \label{fig:circ_asp1}
\end{figure*}
		

Now consider a special case, provided a circle-shape sensor region $\bigcirc_\mathcal{S}$ inside $\bigcirc$ as
$$
\bigcirc_{\mathcal{S}} = \{(x,y)| (x-x_0)^2+(y-y_0)^2 \leq R_2^2\},
$$
where $R_1\geq R_2$, $(x_0,y_0)$ is a known circle center and $R_2$ denotes its radius.



First, choose $O:(x_1,y_1)$ randomly, calculate the $\perp$ cases of a line from $O$ and $\bigcirc_{\mathcal{S}}$ as introduced in Figure
{\small{\begin{equation}
    \begin{aligned}
        & &&(x_{\perp},y_{\perp})\\ 
        &\text{s.t.}&&(x_{\perp}-x_0)^2+(y_{\perp}-y_0)^2 = R_2^2\\
        & &&(x_1-x_0)^2+(y_1-y_0)^2 = (x_{\perp}-x_0)^2+(y_{\perp}-y_0)^2+R_2^2.
    \end{aligned}
\end{equation}}}

% \begin{figure}[t] 
% 	\centering
% 	\includegraphics[width=1\linewidth]{figures/case1.eps}
% 	\caption{Fixed $O$, potential intersection discussion}
% 	\label{fig:1}
% \end{figure}

% \begin{figure}[t] 
% 	\centering
% 	\includegraphics[width=1\linewidth]{figures/case1_2.eps}
% 	\caption{Fixed $O$, potential intersection discussion}
% 	\label{fig:1-1}
% \end{figure}



% \begin{figure}[t] 
% 	\centering
% 	\includegraphics[width=1\linewidth]{figures/case1_OD.eps}
% 	\caption{Fixed $O$, $\Vert OD \Vert_2$ along $\wideparen{D_1 D_2}$}
% 	\label{fig:2}
% \end{figure}


Then, we can calculate the position of $D:(x_2,y_2)$ (two potential cases: $D_1$ and $D_2$) with the possible intersection point of $\bigcirc_{\mathcal{S}}$ and the line of $O\perp$ 
\begin{equation}
    l:\,y = k_1 x +b_1,
\end{equation}
\noindent
where $k_1 =  \frac{y_{\perp}-y_1}{x_{\perp}-x_1}$ and $b_1=\frac{x_{\perp} y_1 - x_1 y_{\perp}}{x_{\perp}- x_1} $ as
{\small{\begin{equation}
    \begin{aligned}
        & &&(x_2,y_2)\\ 
        &\text{s.t.} &&(x_2-x_0)^2+(y_2-y_0)^2 = R_1^2\\
        & &&y_2 = k_1 x_2 +b_1.
    \end{aligned}
\end{equation}}}

The distance of $OD$ can be calculated as
\begin{equation}
    \begin{aligned}
        \Vert OD \Vert_2 = |x_2 -x_1| \sqrt{k^2 +1}.
    \end{aligned}
\end{equation}

The changing tendency of the length of $OD$ along $\wideparen{D_1 D_2}$ sequentially is shown in Figure.

The intersection points of $\bigcirc_{\mathcal{S}}$ and $l$ can be computed as
\begin{equation}\label{eqn:tangentScirc}
        \begin{aligned}
        & &&(x_I,y_I)\\ 
        &\text{s.t.}  &&(x_I-x_0)^2+(y_I-y_0)^2 = R_2^2\\
        & &&y_I = k_2 x_I +b_2.
    \end{aligned}
\end{equation}
\noindent
where $k_2 =  \frac{y_2-y_1}{x_2-x_1}$ and $b_1=\frac{x_2 y_1 - x_1 y_2}{x_2- x_1} $, the point $O(x_1,y_1)$ is still fixed, while $D(x_2,y_2)$ can be any points along $\wideparen{D_1 D_2}$. At this time, we can obtain 2 solutions $I_1, I_2$from (\ref{eqn:tangentScirc}) without that $2$ tangent cases, $x_0,y_0,R_2$ are simplified here, 

{\small{
\begin{equation}\nonumber
    \begin{aligned}
        \begin{bmatrix}
        x_{I_1} = \frac{2\,k_{2}-2\,b_{2}\,k_{2}+\sqrt{2}\,\sqrt{-2\,{b_{2}}^2-4\,b_{2}\,k_{2}+4\,b_{2}-{k_{2}}^2+4\,k_{2}-1}+2}{2\,\left({k_{2}}^2+1\right)} \\
        y_{I_1} = \frac{2\,b_{2}+2\,k_{2}+2\,{k_{2}}^2+\sqrt{2}\,k_{2}\,\sqrt{-2\,{b_{2}}^2-4\,b_{2}\,k_{2}+4\,b_{2}-{k_{2}}^2+4\,k_{2}-1}}{2\,\left({k_{2}}^2+1\right)} 
        \end{bmatrix}
    \end{aligned}
\end{equation}}}
{\small{
\begin{equation}\nonumber
    \begin{aligned}
    \begin{bmatrix}
        x_{I_2} =\frac{2\,k_{2}-2\,b_{2}\,k_{2}+\sqrt{2}\,\sqrt{-2\,{b_{2}}^2-4\,b_{2}\,k_{2}+4\,b_{2}-{k_{2}}^2+4\,k_{2}-1}+2}{2\,\left({k_{2}}^2+1\right)}\\
        y_{I_2} = \frac{2\,b_{2}+2\,k_{2}+2\,{k_{2}}^2-\sqrt{2}\,k_{2}\,\sqrt{-2\,{b_{2}}^2-4\,b_{2}\,k_{2}+4\,b_{2}-{k_{2}}^2+4\,k_{2}-1}}{2\,\left({k_{2}}^2+1\right)} 
        \end{bmatrix}.
    \end{aligned}
\end{equation}}}

% \begin{figure}[t] 
% 	\centering
% 	\includegraphics[width=1\linewidth]{figures/case1_I12.eps}
% 	\caption{Fixed $O$, $\Vert I_1 I_2 \Vert_2$ along $\wideparen{D_1 D_2}$}
% 	\label{fig:3}
% \end{figure}

Thus, we can see the proportion of intersection length and the total length is given in Figure.


% \begin{figure}[t] 
% 	\centering
% 	\includegraphics[width=1\linewidth]{figures/case1_P.eps}
% 	\caption{Fixed $O$, $R_1$, $R_2$, proportion $P$ along $\wideparen{D_1 D_2}$}
% 	\label{fig:4}
% \end{figure}


\begin{figure*}[ht] 
    \centering
    \includegraphics[width=1.0\linewidth]{figures/asp2_demo_circle.eps}
    \caption{Circle case with Assumption 2}
    \label{fig:circ_asp2}
\end{figure*}
		

\begin{figure*}[ht] 
    \centering
    \includegraphics[width=1.0\linewidth]{figures/asp3_demo_circle.eps}
    \caption{Circle case with Assumption 3}
    \label{fig:circ_asp3}
\end{figure*}
		

\begin{figure}[t] 
	\centering
    \includegraphics[width=0.6\linewidth]{figures/circle_sol.png}
    \caption{Circle case Proportion Solution}
    \label{fig:circ_sol}
\end{figure}


\subsection{Case 2: Square Region}

\begin{asu}\label{asu:1}
    The midpoint of the inner chord of a circle are uniformly distributed throughout the interior of the circle.
\end{asu}
\noindent
Accordingly, if there exists a midpoint inside $\mathcal{S}$, the intersection will happen absolutely.



\begin{figure}[t] 
	\centering
    \includegraphics[width=0.6\linewidth]{figures/square_sol.png}
    \caption{Square case Proportion Solution}
    \label{fig:squ_sol}
\end{figure}


According to Assumption \ref{asu:1}, the question about the probability distribution of the intersection proportion can be converged into the probability distribution of a point in radius of $\bigcirc_{\mathcal{S}}$ that works as a midpoint of the string of $\bigcirc_{\mathcal{S}}$ and $\bigcirc$, respectively.

% \begin{figure}[t] 
% 	\centering
% 	\includegraphics[width=1\linewidth]{figures/demonstration.png}
% 	\caption{Another way to consider this question}
% 	\label{fig:5}
% \end{figure}


Link the midpoint with the circle center, the length proportion can be regarded as the area proportion, accordingly as shown in Figure. 

What's more, we can transform the proportion question from mentioned above into the expected distance from the midpoint to the center of the circle. Each midpoint with a fixed distance to the center has a fixed intersection proportion accordingly.

The cumulative distribution function $F(x)$ of the distance $x$ from the midpoint $m$ to the center $G(x_0,y_0)$ is given as 
\begin{equation}
    F(x) = P(X\leq x) = \frac{x^2}{r^2},
\end{equation}
\noindent 
where $r$ denotes the radius of the corresponding circle. Then, the probability density function of $x$ is given as 
\begin{equation}
    p(x) =F'(x)= \frac{2x}{r^2},
\end{equation}
\noindent
while the matching expectation of $d$ is given as 
\begin{equation}
    E[x] =\int_0^r x p(x)  d_x = \frac{2r}{3}.
\end{equation}

Then the intersection proportion $P_{\cap}$ can be calculated as 
\begin{equation}
    P_{\cap} =\frac{\blacktriangle_{\bigcirc_{\mathcal{S}}}}{\blacktriangle_{\bigcirc}}=\frac{l_{\cap}}{l},
\end{equation}
\noindent
where $\blacktriangle_{\bigcirc_{\mathcal{S}}}$ denotes the area of the intersection triangle with $l_{\cap}$ denotes the intersection length, while $\blacktriangle_{\bigcirc}$ denotes the area of the big triangle with $l$ denotes the total length. The formulation of $\blacktriangle_{\bigcirc_{\mathcal{S}}}$ and $\blacktriangle_{\bigcirc}$ are given as
\begin{equation}
    \begin{aligned}
        &\blacktriangle_{\bigcirc_{\mathcal{S}}}&& = \sqrt{ r^2-x^2}\cdot x \cdot 0.5\\
        &\blacktriangle_{\bigcirc}&& =  \sqrt{R^2-x^2}\cdot x \cdot 0.5,
    \end{aligned}
\end{equation}
where the corresponding expectation of $P_{\cap}$ is defined as
\begin{equation}
    \begin{aligned}
        E[P_{\cap}] =  \frac{\sqrt{ r^2-x^2}}{\sqrt{R^2-x^2}}=\frac{\sqrt{ r^2-(E[x])^2}}{\sqrt{R^2-(E[x])^2}}=\frac{\sqrt{5r^2}}{\sqrt{9R^2-4r^2}},
    \end{aligned}
\end{equation}



% \subsection{Case 2: Square Region}
% Given a set $\mathcal{P}$ containing $n$ points in a 2D-plane as 
% $$
% \mathcal{P}=\{(x_1,y_1),(x_2,y_2),\dots,(x_n,y_n)\},
% $$
% while these points are inside a region $\square:[0,l]\times [0,w]$. A special assumption of these points are given here 

% \begin{asu}
%     Points in $\mathcal{P}$ are located at the square boxes uniformly, whose locations are at least either $x=0$ or $y=0$.
% \end{asu}

% Now provided a circle-shape sensor region $\mathcal{S}$ inside $\square$ as
% $$
% \mathcal{S} = \{(x,y)| (x-x_0)^2+(y-y_0)^2 \leq R^2\},
% $$
% where $(x_0,y_0)$ is a known circle center and $R$ denotes its radius.

==> ridcov_atm2023/hh/bak/2_settings.tex <==
\section{Proportion Discussion}\label{SEC_Sets}

We are wondering to estimate the expectation of the length proportion between the crossing length of the sensor area and the total length of each RID in a 2D plane. But before we start, some clarifications need to be stated here. 


Assume there exists two points $A, B$ on the edge of a circle,
$$
\bigcirc\equiv \{(x,y)| (x-x_0)^2+(y-y_0)^2 = R_e^2\},
$$ 
where $(x_0,y_0)=(0,0)$, and the radius of environment $R_e = 1$. We can refer the position of $A, B$ as 
\begin{equation}\label{eq:circ}
    \begin{aligned}
        &A(R_e\cos(\alpha),R_e\sin(\alpha)),\\
        &B(R_e\cos(\beta),R_e\sin(\beta)),
    \end{aligned}
\end{equation}
\noindent
where $\alpha,\beta \sim \mathcal{U}(0,2\pi)$ are the random angles and 
\begin{equation}\label{eq:mid}
    \begin{aligned}
    M(\frac{R_e(\cos(\alpha)+\cos(\beta))}{2},\frac{R_e(\sin(\alpha)+\sin(\beta))}{2}),
    \end{aligned}
\end{equation}
denotes the corresponding midpoint.





The \textbf{coverage estimation} is demonstrated in Figure \ref{fig:prob_circ}, where the ratio between the thicker chord and the thinner chord is the target. Notice that the definition of random select two points on the target square is ambiguous, which is known as the Bertrand Paradox. So, we will give our definitions, methodology and conclusions for RID in this section.

% \begin{figure}[t] 
% 	\centering
% 	\includegraphics[width=1\linewidth]{figures/Rid_coverage_circle_case.eps}
% 	\caption{RID coverage with circle region}
% 	\label{fig:prob_circ}
% \end{figure}


\begin{lem}\label{lem:1}
A chord in the circle can be fixed by finding its midpoint uniquely.
\end{lem}
\noindent
According to Lemma \ref{lem:1}, by linking the midpoint to the circle center, the length coverage can be computed as shown in Figure \ref{fig:prob_circ}, where $P_{\cap} = \frac{L_p}{L}$ denotes the coverage ratio. It means we can reformulate the coverage estimation into the question related to the distance expectation from the midpoint to the center. 

Then the intersection proportion $P_{\cap}$ can be calculated as 
\begin{equation}
    P_{\cap} =\frac{\blacktriangle(\bigcirc_{\mathcal{S}})}{\blacktriangle({\bigcirc})}=\frac{L_{p}}{L},
\end{equation}
\noindent
where $\blacktriangle(\cdot)$ denotes the intersection triangle area, $L_{p}$ and $L$ denote half of the intersection length in $\bigcirc_{S}$ and $\bigcirc$, respectively. Assume the distance from the midpoint to the center is $x$, then we have
\begin{equation}
    \begin{aligned}
        &\blacktriangle(\bigcirc_{\mathcal{S}})&& = \frac{\sqrt{ R_d^2-x^2}\cdot x} {2},\\
        &\blacktriangle({\bigcirc})&& =  \frac{\sqrt{R_e^2-x^2}\cdot x }{2},
    \end{aligned}
\end{equation}
where the corresponding expectation of $P_{\cap}$ is defined as
\begin{equation}\label{eq:exp_cov}
    \begin{aligned}
        P_{\cap} =  \frac{\sqrt{ R_d^2-x^2}}{\sqrt{R_e^2-x^2}}.
    \end{aligned}
\end{equation}
% =\frac{\sqrt{ R_d^2-(E[x])^2}}{\sqrt{R_e^2-(E[x])^2}}

\begin{remark} 
Each chords' midpoint to the center resulting in a fixed intersection proportion, accordingly. But the case of uniform distributed midpoint is different from the uniform distributed starting and ending point of a chord.
\end{remark} 

\subsection{Case 1: Uniformly Distributed Starting and Ending Points}
The starting and ending point are on the edge of $\bigcirc$ in (\ref{eq:circ}), while $\alpha,\beta$ are random variables that are uniformly distributed in the range of $[0,2\pi]$. The position of $M$ is shown in (\ref{eq:mid}). Since the angles $\alpha$ and $\beta$ are distributed uniformly, the result generated from a fixed $\alpha$ is equal to the case of the random selected $\alpha$ in this case.

Assume $\alpha=0$ in Figure \ref{fig:demo_circ}, the midpoint can be obtained from (\ref{eq:mid}) as 
\begin{equation}
    \begin{aligned}
    M(\frac{R_e(1+\cos(\beta))}{2},\frac{R_e\sin(\beta)}{2}),
    \end{aligned}
\end{equation}
\noindent
where the intersection will happen when $\beta\in[\frac{2\pi}{3},\frac{4\pi}{3}]$ in this case. By considering $\beta\sim \mathcal{U}[\frac{2\pi}{3},\frac{4\pi}{3}]$, we can obtain

\begin{equation}
    \begin{aligned}\label{eq:sol_case1}
        & \quad\; x^2 = (\frac{R_e(1+\cos(\beta))}{2})^2+(\frac{R_e\sin(\beta)}{2})^2\\
        & =\frac{R_e^2(1+\cos(\beta))}{2},\\
        & \quad\; E[P^{(1)}_{\cap}] = \frac{4\arcsin(\frac{R_d}{R_e})}{2\pi} E[\sqrt{\frac{R_d^2-x^2}{R_e^2-x^2}}]\\
        &= \frac{4\arcsin(\frac{R_d}{R_e})}{2\pi}  \int_{\pi-2\arcsin(\frac{R_d}{R_e})}^{\pi+2\arcsin(\frac{R_d}{R_e})} \frac{\sqrt{\frac{R_d^2-R_e^2(1+\cos(\beta))/2}{R_e^2-R_e^2(1+\cos(\beta))/2}}}{4\arcsin(\frac{R_d}{R_e})} d \beta,\\
        &\quad\;\beta\in[\pi-2\arcsin(\frac{R_d}{R_e}),\pi+2\arcsin(\frac{R_d}{R_e})],\\
        &\quad\;\cos(\beta)\in[-1,-\cos(2\arcsin(\frac{R_d}{R_e}))],\\
        & \quad\; R_d \in (\frac{\sqrt{2}R_e\sqrt{1+\cos(\beta)}}{2},R_e)=(0,R_e),\\
    \end{aligned}
\end{equation}
% & =\frac{1}{3} \int_{\frac{2\pi}{3}}^{\frac{4\pi}{3}} \frac{3}{2\pi}\sqrt{\frac{R_d^2-R_e^2(1+\cos(\beta))/2}{R_e^2-R_e^2(1+\cos(\beta))/2}} d \beta\\
\noindent
where $E[P^{(1)}_{\cap}]$ denotes the expectation of the trajectory coverage ratio based on the randomly select starting and ending points. When $R_e = 1, R_d = 0.5$, $E[P^{(1)}_{\cap}] \approx 0.13397$.

% Thus, the polynomial fit toward the analytical expression of $P$ within the given range $x = \frac{R_d}{R_e}\in[\frac{1}{2},1]$ can be obtained
% \begin{equation}
%     \begin{aligned}\label{eq:P_case1}
%     P(x)&= \frac{4\arcsin(x)}{2\pi}  \int_{\pi-2\arcsin(x)}^{\pi+2\arcsin(x)} \frac{\sqrt{\frac{2x^2-1-\cos(\beta))}{1-\cos(\beta)}}}{4\arcsin(x)} d \beta\\
%     &=\frac{1}{2\pi} \int_{\pi-2\arcsin(x)}^{\pi+2\arcsin(x)} \sqrt{\frac{2x^2-1-\cos(\beta))}{1-\cos(\beta)}} d \beta. \\
%     \end{aligned}
% \end{equation}

% \begin{figure}[t] 
% 	\centering
% 	\includegraphics[width=1\linewidth]{figures/Rid_case1_alpha0.eps}
% 	\caption{Fixed Starting Point $A$ with $\alpha=0$ for Coverage Ratio Exploration}
% 	\label{fig:demo_circ}
% \end{figure}

 When $R_e$ is defined from $[0.2,2]$ with step $0.2$, we define $R_d=[\frac{R_e}{2},\frac{11R_1}{20},\dots,R_e]$ over the domain, Figure \ref{fig:demo_circle_case}(a) demonstrates these changing.




\begin{figure}
  \centering
  \begin{tabular}{@{}c@{}}
    \includegraphics[width=1\linewidth]{figures/Rid_case1_comp.eps} \\[\abovecaptionskip]
    \small (a) Case 1
  \end{tabular}

  \vspace{\floatsep}

  \begin{tabular}{@{}c@{}}
    \includegraphics[width=1\linewidth]{figures/Rid_case2_comp.eps} \\[\abovecaptionskip]
    \small (b) Case 2
  \end{tabular}

    \caption{Analytical and $10000$ times Monte Carlo Simulation Comparison with Various $R_e-R_d$ pairs of these Case $1,2$.}\label{fig:demo_circle_case}
\end{figure}


\begin{figure}[t] 
	\centering
	\includegraphics[width=1\linewidth]{figures/Rid_case1and2_comp.eps}
	\caption{Circle Cases' comparison}
	\label{fig:demo_circ_comp}
\end{figure}

% Based on case 1, we can obtain any starting and ending points $A,B$ with random variables $\alpha,\beta$ such that
% \begin{equation}
%     \begin{aligned}
%         &x_A = E[\cos(\alpha)]=\int_0^{2\pi}\cos(\alpha)\frac{1}{2\pi}d\alpha =0 \\
%         &y_A = E[\sin(\alpha)]=\int_0^{2\pi}\sin(\alpha)\frac{1}{2\pi}d\alpha=0\\
%         &x_B = E[\cos(\beta)]=\int_0^{2\pi}\cos(\beta)\frac{1}{2\pi}d\beta =0\\
%         &y_B =E[\sin(\beta)]=\int_0^{2\pi}\sin(\beta)\frac{1}{2\pi}d\beta=0.
%     \end{aligned}
% \end{equation}

\subsection{Case 2: Uniformly Distributed Midpoint}

The CDF $F(y)$ of the distance $y$ from the midpoint $m(x_m,y_m)$ to the center $O$ is 
\begin{equation}
    F(y) = P(Y\leq y) = \frac{\pi y^2}{\pi R_e^2},\quad y\in[0,R_e].
\end{equation}
\noindent 
Then, the PDF of $y$ is given as 
\begin{equation}\label{eq:exp_case2}
    f_Y(y) =F'(y)= 
    \left\{
    \begin{aligned}
    &\frac{2y}{R_e^2}\quad &&y\in[0,R_e],\\
    & 0 && \text{otherwise}.
    \end{aligned}
    \right.
\end{equation}

Therefore, based on (\ref{eq:exp_cov}) and (\ref{eq:exp_case2}), we can compute the expectation of the coverage proportion as
\begin{equation}\label{eq:sol_case2}
    \begin{aligned}
    E[P^{(2)}_{\cap}] &= E[\sqrt{\frac{R_d^2-y^2}{R_e^2-y^2}}]\\
    &= \int_0^{R_d}\sqrt{\frac{R_d^2-y^2}{R_e^2-y^2}}f_Y(y)dy+\int_{R_d}^{R_e}0 f_Y(y)dy\\
    &= \int_0^{R_d}\sqrt{\frac{R_d^2-y^2}{R_e^2-y^2}}\frac{2y}{R_e^2}dy\\
    & R_d\in(0,R_e),
    \end{aligned}
\end{equation}
\noindent
where $E[P^{(2)}_{\cap}]$ denotes the expectation of the trajectory coverage ratio based on the randomly select midpoints. When $R_e = 1, R_d = 0.5$, $E[P^{(2)}_{\cap}] \approx 0.0884$. When $R_e$ is defined from $[0.2,2]$ with step $0.2$, we define $R_d=[\frac{R_e}{10},\frac{2R_1}{10},\dots,R_e]$ over the domain, Figure \ref{fig:demo_circle_case}(b) demonstrates these changing.





% Thus, the polynomial fit toward the analytical expression of $P$ within the given range $x = \frac{R_d}{R_e}\in(0,1)$ can be obtained
% \begin{equation}
%     \begin{aligned}\label{eq:P_case2}
%     P(x)&= \int_0^{R_d}\sqrt{\frac{x^2-(\frac{y}{R_e})^2}{1-(\frac{y}{R_e})^2}}\frac{2y}{R_e^2}dy.\\
%     \end{aligned}
% \end{equation}

% Based on case 2, we can obtain any starting and ending points $A,B$ with random variables $\alpha,\beta$ such that
% \begin{equation}
%     \begin{aligned}
%         &x_A = E[\cos(\alpha)]=\int_0^{2\pi}\cos(\alpha)\frac{1}{2\pi}d\alpha =0 \\
%         &y_A = E[\sin(\alpha)]=\int_0^{2\pi}\sin(\alpha)\frac{1}{2\pi}d\alpha=0\\
%         &x_B = E[\cos(\beta)]=\int_0^{2\pi}\cos(\beta)\frac{1}{2\pi}d\beta =0\\
%         &y_B =E[\sin(\beta)]=\int_0^{2\pi}\sin(\beta)\frac{1}{2\pi}d\beta=0.
%     \end{aligned}
% \end{equation}

The difference between (\ref{eq:sol_case1}) and (\ref{eq:sol_case2}) is because the midpoints are satisfied in a different distribution as shown in Figure \ref{fig:midpoint_comp}. Midpoints are uniformly distributed in the left scheme of Figure \ref{fig:midpoint_comp}, which is an ideal state. When we considered the RID are from different direction uniformly, the corresponding trajectories' midpoints should be dense at the origin, which is more realistic and reasonable. Based on the previous result, we can also declare that the coverage ratio's expectation along a square's edge (not a circle's edge) will be close to the circle case because of the symmetry.


% \begin{figure}[t] 
% 	\centering
% 	\includegraphics[width=1\linewidth]{figures/Rid_midpoints_dist.eps}
% 	\caption{Midpoints' Distribution for $(a)$ Case 1 and $(b)$ Case 2}
% 	\label{fig:midpoint_comp}
% \end{figure}



\begin{figure}[t] 
	\centering
	\includegraphics[width=1\linewidth]{figures/Rid_intersect.eps}
	\caption{Monte Carlo Simulation Result of these $2$ Cases}
	\label{fig:demo_mc}
\end{figure}




==> ridcov_atm2023/hh/bak/2_settings_bak.tex <==
\section{Proportion Discussion}\label{SEC_Sets}

We are wondering to estimate the expectation of the length proportion between the crossing length of the sensor area and the total length of each RID in a 2D plane. But before we start, some clarifications need to be stated here. 


Assume there exists two points $A, B$ on the edge of a circle,
$$
\bigcirc\equiv \{(x,y)| (x-x_0)^2+(y-y_0)^2 = R_1^2\},
$$ 
where $(x_0,y_0)=(0,0), R_1 = 1$ for simplicity. We can refer the position of $A, B$ as 
\begin{equation}\label{eq:circ}
    \begin{aligned}
        &A(\cos(\alpha),\sin(\alpha)),\\
        &B(\cos(\beta),\sin(\beta)),
    \end{aligned}
\end{equation}
\noindent
where $\alpha,\beta \sim \mathcal{U}(0,2\pi)$ are the random angles and 
\begin{equation}\label{eq:mid}
    \begin{aligned}
    M(\frac{\cos(\alpha)+\cos(\beta)}{2},\frac{\sin(\alpha)+\sin(\beta)}{2}),
    \end{aligned}
\end{equation}
denotes the corresponding midpoint.



Now consider a special circle-shape sensor region $\bigcirc_\mathcal{S}$
$$
\bigcirc_{\mathcal{S}} = \{(x,y)| (x-x_0)^2+(y-y_0)^2 \leq R_2^2\},
$$
where $R_2=0.5$ in this case.

The \textbf{coverage estimation} is demonstrated in Figure \ref{fig:prob_circ}, where the ratio between the thicker chord and the thinner chord is the target. Notice that the definition of random select two points on the target square is ambiguous, which is known as the Bertrand Paradox. So, we will give our definitions, methodology and conclusions for RID in this section.

\begin{figure}[t] 
	\centering
	\includegraphics[width=1\linewidth]{figures/prob_demo_circle.eps}
	\caption{RID coverage with circle region}
	\label{fig:prob_circ}
\end{figure}

\begin{figure}[t] 
	\centering
    \includegraphics[width=0.6\linewidth]{figures/circle_sol.png}
    \caption{Circle case Proportion Solution}
    \label{fig:circ_sol}
\end{figure}


\begin{lem}\label{lem:1}
A chord in the circle can be fixed by finding its midpoint uniquely.
\end{lem}
\noindent
According to Lemma \ref{lem:1}, by linking the midpoint to the circle center, the length coverage can be computed as shown in Figure \ref{fig:circ_sol}, where $P_{\cap} = \frac{L_p}{L}$ denotes the coverage ratio. It means we can reformulate the coverage estimation into the question related to the distance expectation from the midpoint to the center. 

Then the intersection proportion $P_{\cap}$ can be calculated as 
\begin{equation}
    P_{\cap} =\frac{\blacktriangle(\bigcirc_{\mathcal{S}})}{\blacktriangle({\bigcirc})}=\frac{L_{p}}{L},
\end{equation}
\noindent
where $\blacktriangle(\cdot)$ denotes the intersection triangle area, $L_{p}$ and $L$ denote half of the intersection length in $\bigcirc_{S}$ and $\bigcirc$, respectively. Assume the distance from the midpoint to the center is $x$, then we have
\begin{equation}
    \begin{aligned}
        &\blacktriangle(\bigcirc_{\mathcal{S}})&& = \frac{\sqrt{ R_2^2-x^2}\cdot x} {2},\\
        &\blacktriangle({\bigcirc})&& =  \frac{\sqrt{R_1^2-x^2}\cdot x }{2},
    \end{aligned}
\end{equation}
where the corresponding expectation of $P_{\cap}$ is defined as
\begin{equation}\label{eq:exp_cov}
    \begin{aligned}
        P_{\cap} =  \frac{\sqrt{ R_2^2-x^2}}{\sqrt{R_1^2-x^2}}.
    \end{aligned}
\end{equation}
% =\frac{\sqrt{ R_2^2-(E[x])^2}}{\sqrt{R_1^2-(E[x])^2}}

\begin{remark} 
Each chords' midpoint to the center resulting in a fixed intersection proportion, accordingly. But the case of uniform distributed midpoint is different from the uniform distributed starting and ending point of a chord.
\end{remark} 

\subsection{Case 1: Uniformly Distributed Starting and Ending Points}
The starting and ending point are on the edge of $\bigcirc$ in (\ref{eq:circ}), while $\alpha,\beta$ are random variables that are uniformly distributed in the range of $[0,2\pi]$. The position of $M$ is shown in (\ref{eq:mid}). We can reformulate (\ref{eq:mid}) to obtain
\begin{equation}\label{eq:exp_rsep}
    \begin{aligned}
     M(\underbrace{\cos(\frac{\alpha+\beta}{2})}_{\text{Term 1}}\cos(\frac{\alpha-\beta}{2}),\underbrace{\sin(\frac{\alpha+\beta}{2})}_{\text{Term 2}}\underbrace{\cos(\frac{\alpha-\beta}{2}))}_{\text{Term 3}}.
    \end{aligned}
\end{equation}

Since $\alpha,\beta$ are independent, their joint distribution is
\begin{equation}
    f(\alpha,\beta) = \left\{ 
    \begin{aligned}
        &\frac{1}{4\pi^2} \quad && \alpha\in[0,2\pi],\beta\in[0,2\pi],\\
        &0 && \text{otherwise}.
    \end{aligned}
    \right.
\end{equation}
\noindent
Assume $z_1 = \frac{\alpha+\beta}{2}$, we can obtain the Jacobian matrix $J$ from
\begin{equation}
    \begin{aligned}
        &0 \leq && t_1= \alpha &&\leq 2\pi,\\
        &0 \leq && t_2= 2Z - \alpha &&\leq 2\pi,
    \end{aligned}
\end{equation}

\noindent
as $J_1 = \begin{vmatrix}
    \frac{\partial t_1}{\partial \alpha}&\frac{\partial t_1}{\partial z_1}\\
    \frac{\partial t_2}{\partial \alpha}&\frac{\partial t_2}{\partial z_1}
\end{vmatrix} = 
\begin{vmatrix}
    1&0\\-1&2
\end{vmatrix}$ and $|J_1| = 2$. Then, formulate $z_1$ probability density function (PDF) as
\begin{equation}
    \begin{aligned}
    f_{Z_1}(z_1) =\left\{ 
    \begin{aligned}
        &\int_{0}^{2z_1} \frac{2}{4\pi^2}d \alpha= \frac{z_1}{\pi^2} &&z_1\in[0,\pi),\\
        &\int_{2z_1 - 2\pi}^{2\pi} \frac{2}{4\pi^2}d \alpha= \frac{2\pi - z_1}{\pi^2} &&z_1\in[\pi,2\pi],\\
        & 0 && \text{otherwise}.
    \end{aligned}
    \right.
    \end{aligned}
\end{equation}

\noindent 
Thus, we have the cumulative density function (CDF) of $z_1$,
\begin{equation}
    \begin{aligned}
    F(z_1) =\left\{ 
    \begin{aligned}
        & 0 &&z_1\in(-\infty,0),\\
        &\frac{z_1^2}{2\pi^2} &&z_1\in[0,\pi),\\
        &\frac{2z_1}{\pi}-\frac{z^2_1}{2\pi^2}-1 &&z_1\in[\pi,2\pi],\\
        & 1 &&z_1\in(2\pi,\infty).\\
    \end{aligned}
    \right.
    \end{aligned}
\end{equation}

\subsubsection{Term 1}
\noindent 
Defining $u = U = \cos(z_1)$, and $z_1 = \arccos (u), u\in[-1,1]$ 
$$
\frac{d z_1}{d u}=-\frac{1}{\sqrt{1-u^2}}.
$$ 
The CDF of $u$ is obtained as
\begin{equation}
    \begin{aligned}
    F(u) &= P\{ U\leq u \} = P\{\cos(z_1)\leq u\}\\
    &= P\{\arccos(u)\leq z_1 \leq 2\pi-\arccos(u)\}\\
    &= \frac{2(2\pi - \arccos(u))}{\pi}-\frac{(2\pi - \arccos(u))^2}{2\pi^2}\\
    &\quad -1-\frac{(\arccos(u))^2}{2\pi^2}\\
    &= \frac{\pi^2-(\arccos(u))^2}{\pi^2}.
    \end{aligned}
\end{equation}
\noindent
Thus, the corresponding PDF of $u$ is 
\begin{equation}
    \begin{aligned}
    f_{U}(u) =\left\{ 
    \begin{aligned}
        & \frac{2 \arccos(u)}{\pi^2 \sqrt{1-u^2}} &&u\in[-1,1]\\
        &0 && \text{otherwise}.
    \end{aligned}
    \right.
    \end{aligned}
\end{equation}
\noindent
The corresponding expectation of $u$ can be computed as
\begin{equation}
    \begin{aligned}\label{eq:exp_u}
        \mathbf{E}[u] =\mathbf{E}[\cos(\frac{\alpha+\beta}{2})]= \int_{-1}^1 u f_U(u) du = -0.4053.
    \end{aligned}
\end{equation}

\subsubsection{Term 2}
Next, defining $v = V = \sin(z_1)$, and $z_1 = \arcsin (v), v\in[-1,1]$ that 
$$
\frac{d z_1}{d v}=\frac{1}{\sqrt{1-v^2}}.
$$ 
The CDF of $v$ is obtained as
\begin{equation}
    \begin{aligned}
    F(v) &= P\{ V\leq v \} = P\{\sin(z_1)\leq v\}\\
    &= P\{z_1\leq \arcsin(v)\\
    &=\left\{ 
    \begin{aligned}
        & 0 &&\quad \,z_1\in(-\infty,0),\\
        & P\{z_1\leq \arcsin(v)\}+&&\\
        & \quad P\{z_1\geq \pi - \arcsin(v)\} &&\quad \, z_1\in[0,\pi],\\
        & P\{\pi - \arcsin(v) \leq z_1 \leq &&\\
        & \quad 2\pi+\arcsin(v)\} &&\quad \,z_1\in[\pi,2\pi],\\
        & 1 &&\quad \, z_1\in(2\pi,\infty).\\
    \end{aligned}
    \right.\\
    &=\left\{ 
    \begin{aligned}
        & 0 &&v\in(-\infty,-1),\\
        & \frac{\pi^2+2\pi \arcsin(v)}{2\pi^2} &&v\in[-1,1],\\
        & 1 &&v\in(1,\infty).\\
    \end{aligned}
    \right.
    \end{aligned}
\end{equation}

\noindent
Thus, the corresponding PDF of $v$ is 
\begin{equation}
    \begin{aligned}
    f_{V}(v) =\left\{ 
     \begin{aligned}
        & \frac{1}{\pi \sqrt{1-v^2}} &&v\in[-1,1],\\
        &0 && \text{otherwise}.
    \end{aligned}
    \right.
    \end{aligned}
\end{equation}
\noindent
The corresponding expectation of $v$ can be computed as
\begin{equation}
    \begin{aligned}\label{eq:exp_v}
        \mathbf{E}[v] =\mathbf{E}[\sin(\frac{\alpha+\beta}{2})] = \int_{-1}^1 v f_V(v) dv = 0.
    \end{aligned}
\end{equation}


\subsubsection{Term 3}
Defining $z_2 = \frac{\alpha-\beta}{2}$, $w = W = \cos(z_2)$ and $\beta = \alpha - 2z_2$. We can obtain the Jacobian matrix $J_2$ from
\begin{equation}
    \begin{aligned}
        &0 \leq && t_3= \alpha &&\leq 2\pi,\\
        &0 \leq && t_4= \alpha - 2z_2 &&\leq 2\pi,
    \end{aligned}
\end{equation}

\noindent
as $J_2 = \begin{vmatrix}
    \frac{\partial t_3}{\partial \alpha}&\frac{\partial t_3}{\partial z_1}\\
    \frac{\partial t_4}{\partial \alpha}&\frac{\partial t_4}{\partial z_1}
\end{vmatrix} = 
\begin{vmatrix}
    1&0\\1&-2
\end{vmatrix}$ and $|J_2| = 2$. Then, formulate $z_2$ PDF as
\begin{equation}
    \begin{aligned}
    f_{Z_2}(z_2) =\left\{ 
    \begin{aligned}
        &\int_{0}^{2z_2+2\pi} \frac{2}{4\pi^2}d \alpha = \frac{\pi+z_2}{\pi^2} &&z_2\in[-\pi,0),\\
        &\int_{2z_2 }^{2\pi}  \frac{2}{4\pi^2} d \alpha = \frac{\pi-z_2}{\pi^2}&&z_2\in[0,\pi],\\
        & 0 && \text{otherwise}.
    \end{aligned}
    \right.
    \end{aligned}
\end{equation}

\noindent 
Thus, we have the CDF of $z_2$,
\begin{equation}
    \begin{aligned}
    F(z_2) =\left\{ 
    \begin{aligned}
        & 0 &&z_2\in(-\infty,-\pi),\\
        &\frac{2\pi z_2+z^2_2}{2\pi^2} &&z_2\in[-\pi,0),\\
        &\frac{2\pi z_2-z^2_2}{2\pi^2} &&z_2\in[0,\pi],\\
        & 1 &&z_2\in(\pi,\infty).\\
    \end{aligned}
    \right.
    \end{aligned}
\end{equation}

\noindent 
Defining $w = W = \cos(z_2)$, and $z_2 = \arccos (w), w\in[-1,1]$, we can obtain
$$
\frac{d z_2}{d w}=-\frac{1}{\sqrt{1-w^2}}.
$$ 
The CDF of $w$ is obtained as
\begin{equation}
    \begin{aligned}
    F(w) &= P\{ W\leq w \} = P\{\cos(z_2)\leq w\}\\
    &= P\{z_2\leq -\arccos(w)\}+ P\{z_2\geq \arccos(w)\}\\
    &= 1 - P\{-\arccos(w)\leq z_2 \leq \arccos(w) \}\\
    &= 1 - \frac{2\arccos(w)}{\pi}+\frac{(\arccos(w))^2}{\pi^2}.
    \end{aligned}
\end{equation}
\noindent
Thus, the corresponding PDF of $w$ is 
\begin{equation}
    \begin{aligned}
    f_{W}(w) =\left\{ 
    \begin{aligned}
        & \frac{2}{\pi \sqrt{1-w^2}}- \frac{2\arccos(w)}{\pi^2\sqrt{1-w^2}} &&w\in[-1,1]\\
        &0 && \text{otherwise}.
    \end{aligned}
    \right.
    \end{aligned}
\end{equation}
\noindent
The corresponding expectation of $w$ can be computed as
\begin{equation}\label{eq:exp_w}
    \begin{aligned}
        \mathbf{E}[w] =\mathbf{E}[\cos(\frac{\alpha-\beta}{2})]= \int_{-1}^1 w f_W(w) dw = 0.4053.
    \end{aligned}
\end{equation}


% \subsubsection{Length Coverage Expectation in Case 1}

% Assume $\alpha=0$ as shown in Figure \ref{fig:demo_circ}, $\beta\sim \mathcal{U} [0,2\pi]$. The midpoint can be obtained from (\ref{eq:exp_rsep}) as 
% \begin{equation}
%     \begin{aligned}
%     M(\frac{1+\cos(\beta)}{2},\frac{\sin(\beta)}{2}),
%     \end{aligned}
% \end{equation}
% \noindent
% where the intersection will happen when $\beta\in[\frac{5\pi}{6},\frac{7\pi}{6}]$.


% \begin{figure}[t] 
% 	\centering
% 	\includegraphics[width=1\linewidth]{figures/asp1_demo.eps}
% 	\caption{Fixed Starting Point $A$ with $\alpha=0$ for Coverage Ratio Exploration}
% 	\label{fig:demo_circ}
% \end{figure}


\subsection{Case 2: Uniformly Distributed Midpoint}

The CDF $F(x)$ of the distance $x$ from the midpoint $m(x_m,y_m)$ to the center $O$ is 
\begin{equation}
    F(x) = P(X\leq x) = \frac{\pi x^2}{\pi R_1^2},\quad x\in[0,R_1].
\end{equation}
\noindent 
Then, the PDF of $x$ is given as 
\begin{equation}\label{eq:exp_case2}
    f_X(x) =F'(x)= 
    \left\{
    \begin{aligned}
    &\frac{2x}{R_1^2}\quad &&x\in[0,R_1],\\
    & 0 && \text{otherwise},
    \end{aligned}
    \right.
\end{equation}
\noindent
whose expectation is given as 
\begin{equation}
    E[x] =\int_0^{R_1} x f_X(x)  dx = \frac{2R_1}{3}.
\end{equation}

% Defining $k = x^2, x\in[0,\sqrt{R_1}]$, we can obtain
% \begin{equation}
%     f_K(k) = 
%     \left\{
%     \begin{aligned}
%     &1\quad &&k\in[0,R_1],\\
%     & 0 && \text{otherwise},
%     \end{aligned}
%     \right.
% \end{equation}

% \noindent
% whose expectation is given as 
% \begin{equation}
%     E[k] = E[x^2]=\int_0^{R_1} k f_K(k)  dk = \frac{R^2_1}{2}.
% \end{equation}

% However, to describe the event $A,B$ intersected $\bigcirc_S$, a conditional probability need to be added to the uniform distributed midpoint assumption, that the qualified midpoints should be located in $\bigcirc_S$, which results in 
% \begin{equation}\label{eq:exp_case2}
%     E[\Bar{k}] = \int_0^{R_2} k f_K(k)  dk = \frac{R_2^2}{2},
% \end{equation}
% \noindent
% where $\Bar{k}$ denotes the case that if intersect happens, the distance's square expectation from the uniformly selected midpoint to the center.

Therefore, based on (\ref{eq:exp_cov}) and (\ref{eq:exp_case2}), we can compute the expectation of the coverage proportion as
\begin{equation}\label{eq:sol_case2}
    \begin{aligned}
    E[P_{\cap}] &= \frac{\pi R_2^2}{\pi R_1^2} E[\sqrt{\frac{R_2^2-x^2}{R_1^2-x^2}}]\\
    &= \frac{1}{4}\int_0^{R_2}\sqrt{\frac{R_2^2-x^2}{R_1^2-x^2}}f_X(x)dx\\
    &\approx 0.022,
    \end{aligned}
\end{equation}
\noindent
where $E[P_{\cap}]$ denotes the expectation of the trajectory coverage ratio based on the randomly select midpoints.


==> ridcov_atm2023/hh/bak/3_random_cut.tex <==
\section{Random Cut}\label{SEC_Cuts}




\begin{figure}[t] 
	\centering
	\includegraphics[width=1\linewidth]{figures/random_cut.eps}
	\caption{Different Linkage with a pair of fixed starting and ending points}
	\label{fig:demo_cut}
\end{figure}

==> ridcov_atm2023/hh/bak/4_square_case.tex <==
\section{Square Case}\label{SEC_Square}

We demonstrate the situations for the square environment in this section. Defining the square has $4$ sides, with $1,2,3,4$ respectively. If we randomly select the starting and ending point from these $4$ sides, we will generate the combination $C^{\square}$ as shown below
$$
C^{\square} = 
\begin{bmatrix}
(1,1)&(1,2)&(1,3)&(1,4)\\
(2,1)&(2,2)&(2,3)&(2,4)\\
(3,1)&(3,2)&(3,3)&(3,4)\\
(4,1)&(4,2)&(4,3)&(4,4)\\
\end{bmatrix},
$$
where these points' selection can be divided into three categories, both on the same side, on the adjacent side and on the opposite side. This means we only need to compute the expectation of these three kinds of RID, and plug into the relationship table above, then we can obtain the corresponding proportion expectation.

\subsection{Adjacent Side Selection}
Assume the figure are shown in the figure below, assume the starting point $P$ in side $1$ is fixed with $x=0$. And its $y$ value is uniformly distributed as $y\sim \mathcal{U}(0,2d)$, where $L=2d$ denotes the total length of the side. The ending point $Q$ can be fixed in $2$ side, which means its $y$ value is fixed as $2d$ while its $x$ value is uniformly distributed $x\sim\mathcal{U}(0,2d)$. Therefore, we obtain 
$$
\begin{aligned}
&P(0,y),\quad &&y\sim\mathcal{U}(0,2d)\\
&Q(x,2d),\quad &&x\sim\mathcal{U}(0,2d).
\end{aligned}
$$

We can obtain that the tangent case happen when
$$
y = 2d(1-\frac{1}{\tan(\frac{\pi}{4}+\arcsin(\frac{R_d}{\sqrt{2d}}))}).
$$
And we can also obtain the tangent case happen with certain $x$ value in this situation that
$$
x = \frac{d(d-y)(2d-y)-\sqrt{d^2(y-d)^2(2d-y)^2-((d-y)^2-R_d^2)(2d-y)^2(d^2-R_d^2)}}{2((d-y)^2-R_d^2)}
$$
and the corresponding proportion of each $x$ is

$$
P = \frac{\sqrt{{\left(2\,d+2\,k\,\left(d+\left(d-k\,\left(b-d\right)\right)\,\left(k^2+1\right)\right)\right)}^2-\left(2\,k^2+2\right)\,\left({\left(3\,d+2\,k\,\left(d+\left(d-k\,\left(b-d\right)\right)\,\left(k^2+1\right)\right)\right)}^2+d^2-r^2\right)}}{x(k^2+1)}
$$
where 
$$
\begin{aligned}
    &k = \frac{2d-y}{x}\\
    &b = y.
\end{aligned}
$$
Therefore, we can obtain $P$ at each $x,y$ in the following form

$$
P = \frac{\sqrt{{\left(2\,d+\frac{2\,\left(3\,d+\frac{2\,\left(d+\left(d+\frac{\left(d-y\right)\,\left(2\,d-y\right)}{x}\right)\,\left(\frac{{\left(2\,d-y\right)}^2}{x^2}+1\right)\right)\,\left(2\,d-y\right)}{x}\right)\,\left(2\,d-y\right)}{x}\right)}^2-\left(\frac{2\,{\left(2\,d-y\right)}^2}{x^2}+2\right)\,\left({\left(3\,d+\frac{2\,\left(3\,d+\frac{2\,\left(d+\left(d+\frac{\left(d-y\right)\,\left(2\,d-y\right)}{x}\right)\,\left(\frac{{\left(2\,d-y\right)}^2}{x^2}+1\right)\right)\,\left(2\,d-y\right)}{x}\right)\,\left(2\,d-y\right)}{x}\right)}^2+d^2-r^2\right)}}{x\,\left(\frac{{\left(2\,d-y\right)}^2}{x^2}+1\right)}
$$
And when we replace $x$ with $y$, we can see

$$
P = \frac{\left(r^2-{\left(d-y\right)}^2\right)\,\sqrt{{\left(2\,d+\frac{2\,\left(d+\left(d+\frac{\left(d-y\right)\,\left(2\,d-y\right)}{x}\right)\,\left(\frac{{\left(2\,d-y\right)}^2}{x^2}+1\right)\right)\,\left(2\,d-y\right)}{x}\right)}^2-\left(\frac{2\,{\left(2\,d-y\right)}^2}{x^2}+2\right)\,\left({\left(3\,d+\frac{2\,\left(d+\left(d+\frac{\left(d-y\right)\,\left(2\,d-y\right)}{x}\right)\,\left(\frac{{\left(2\,d-y\right)}^2}{x^2}+1\right)\right)\,\left(2\,d-y\right)}{x}\right)}^2+d^2-r^2\right)}}{\left(\sqrt{d^2\,{\left(d-y\right)}^2\,{\left(2\,d-y\right)}^2+\left(d^2-r^2\right)\,\left(r^2-{\left(d-y\right)}^2\right)\,{\left(2\,d-y\right)}^2}-d\,\left(d-y\right)\,\left(2\,d-y\right)\right)\,\left(\frac{{\left(2\,d-y\right)}^2}{x^2}+1\right)}
$$

At this time, to compute the proportion 

\begin{figure}[t] 
	\centering
	\includegraphics[width=1\linewidth]{figures/prob_demo_square.eps}
	\caption{RID coverage with square region}
	\label{fig:prob_squ}
\end{figure}

\begin{figure}[t] 
	\centering
    \includegraphics[width=0.6\linewidth]{figures/square_sol.png}
    \caption{Square case Proportion Solution}
    \label{fig:squ_sol}
\end{figure}


==> ridcov_atm2023/hh/modification.tex <==
% 2023.01.31 Tuesday Meeting with Billy and Max
% Fixed 
% {
%  fig1: legend -- Be - Dc
%  fig2: legend blue line: no coverage
%  fig3: fine
%  fig4: (a) Y lable: E[P_{UDE}]; legend: Eqn. (4), red line: MC, \bc 1\sigma
%       (b) Y lable: E[P_{UDM}]: legend: Eqn. (4), red line: MC, \bc 1\sigma
%  fig5: X label $\rho$
% }

% Unfinished 
% proof: try to generate math proof without mathematical statement
